Exploring the Landscape of Text-to-SQL with Large Language Models: Progresses, Challenges and Opportunities

Converting natural language (NL) questions into SQL queries, referred to as Text-to-SQL, has emerged as a pivotal technology for facilitating access to relational databases, especially for users without SQL knowledge. Recent progress in large language models (LLMs) has markedly propelled the field of natural language processing (NLP), opening new avenues to improve text-to-SQL systems. This study presents a systematic review of LLM-based text-to-SQL, focusing on four key aspects: (1) an analysis of the research trends in LLM-based text-to-SQL; (2) an in-depth analysis of existing LLM-based text-to-SQL techniques from diverse perspectives; (3) summarization of existing text-to-SQL datasets and evaluation metrics; and (4) discussion on potential obstacles and avenues for future exploration in this domain. This survey seeks to furnish researchers with an in-depth understanding of LLM-based text-to-SQL, sparking new innovations and advancements in this field.

==> Table/1.tex <==
\begin{figure}
\centering 
\begin{tikzpicture}[
  grow=right,
  level 1/.style={sibling distance=60mm, level distance=30mm}, 
  edge from parent/.style={-,draw},
  >=latex,
  edge from parent path={(\tikzparentnode.south) -- ++(0:1mm) -- (\tikzchildnode.north)}
]

% 根节点
\node[root,rotate=90] (a1){Ways of Organizing Surveyed Articles} ;

\begin{scope}[every node/.style={level 9}]
\node [right of = a1, node distance=10mm, yshift=53mm, rotate=90] (k1) {Methodologies};  
\node [right of = a1, node distance=10mm, yshift=-51mm, rotate=90] (k2) {Benchmarks}; 
\end{scope} 

\begin{scope}[every node/.style={level 2}]
\node [right of = k1, node distance=0mm, yshift=-55mm, rotate=90] (c1) {Post-Processing};  % 正右边
\node [right of = k1, node distance=0mm, rotate=90] (c2) {Text-to-SQL \\Translation}; 
\node [right of = k1, node distance=0mm, yshift=45mm, rotate=90] (c3) {Pre-Processing}; % 右上方
\end{scope} 

\begin{scope}[every node/.style={level 2}]
\node [right of = k2, node distance=0mm, yshift=17mm, rotate=90] (l1) {Datasets};  % 正右边
\node [right of = k2, node distance=0mm, yshift=-13mm, rotate=90] (l2) {Evaluation Metrics}; 
\end{scope} 

\begin{scope}[every node/.style={level 3}]
\node [right of = c2, node distance=13mm, yshift=11mm, rotate=90] (c21) {In-Context Learning};  % 正右边
\node [right of = c2, node distance=13mm, yshift=-19mm, rotate=90] (c22) {Fine-Tuning}; % 右上方
\end{scope}  

% 第二级的子节点，进一步增加垂直和水平偏移
\begin{scope}[every node/.style={level 4}]
\node [right of = l1, node distance=20mm, yshift=14mm] (l11) {Single-Domain};  
\node [right of = l1, node distance=20mm, yshift=6mm] (l12) {Cross-Domain}; 
\node [right of = l1, node distance=20mm, yshift=-2mm] (l13) {Context-Dependent};
\node [right of = l1, node distance=20mm, yshift=-10mm] (l14) {Cross-Lingual};
\node [right of = l1, node distance=20mm, yshift=-18mm] (l15) {Robustness-Centered};  

\node [right of = l2, node distance=20mm, yshift=4mm] (l21) {Content Matching-based};  % 正右边
\node [right of = l2, node distance=20mm, yshift=-4mm] (l22) {Execution Result-based}; % 右上方

\node [right of = c1, node distance=20mm] (c11) {Execution-Guided SQL Correction};  % 正右边
\node [right of = c1, node distance=20mm, , yshift=9mm] (c12) {Direct SQL \\ Correction}; % 右上方
\node [right of = c1, node distance=20mm, yshift=-9mm] (c13) {Output \\Consistency}; % 右下方

\node [right of = c3, node distance=20mm, yshift=14mm] (c31) {Schema linking};  
\node [right of = c3, node distance=20mm, yshift=5mm] (c32) {Database Content Acquisition}; 
\node [right of = c3, node distance=20mm, yshift=-4mm] (c33) {Question Rewriting};
\node [right of = c3, node distance=20mm, yshift=-13mm] (c34) {Data Augmentation};

\node [right of = c21, node distance=20mm, yshift=10mm] (b2) {Supplementary Knowledge \\Incorporation}; 
\node [right of = c21, node distance=20mm] (b3) {Example Selection};
\node [right of = c21, node distance=20mm, yshift=-10mm] (b4) {Reasoning \\Enhancement};

\node [right of = c22, node distance=20mm, yshift=10mm] (d1) {Novel Model \\Architectures}; 
\node [right of = c22, node distance=20mm ] (d2) {Selection of \\Open-Source Models};
\node [right of = c22, node distance=20mm, yshift=-14mm] (d3) {Model Training};

\end{scope}

\begin{scope}[every node/.style={level 10}]
\node [right of = d3, node distance=22mm, yshift=3.5mm] (e51) {FFT}; 
\node [right of = d3, node distance=22mm, yshift=-4.5mm] (e52) {PEFT}; 
\end{scope}

\begin{scope}[every node/.style={level 5}]
\node [right of = c11, node distance=53mm] (c111) {};  
\node [right of = c12, node distance=53mm] (c122) {};

\node [right of = c13, node distance=53mm] (c133) {}; 

\node [right of = c31, node distance=53mm] (c311) {};  
\node [right of = c32, node distance=53mm] (c322) {};
\node [right of = c33, node distance=53mm] (c333) {}; 
\node [right of = c34, node distance=53mm] (c344) {};  

\node [right of = b2, node distance=53mm] (b22) {};

\node [right of = b3, node distance=53mm] (b33) {};

\node [right of = b4, node distance=53mm] (b44) {};

\node [right of = d1, node distance=53mm] (d11) {};
\node [right of = d2, node distance=53mm] (d12) {}; 

\node [right of = e51, node distance=41mm] (d21) {};
\node [right of = e52, node distance=41mm] (d22) {};

\node [right of = l11, node distance=53mm] (l111) {};
\node [right of = l12, node distance=53mm] (l122) {};
\node [right of = l13, node distance=53mm] (l133) {};
\node [right of = l14, node distance=53mm] (l144) {};
\node [right of = l15, node distance=53mm] (l155) {};

\node [right of = l21, node distance=53mm] (l211) {};
\node [right of = l22, node distance=53mm] (l222) {};
\end{scope}

% 连接每个第一级节点与它的子节点
\foreach \value in {1,2}
  \draw[-] (a1.south) -| ++(1.5mm,0)|- (k\value.north);

\foreach \value in {1,2,3}
  \draw[-] (k1.south) -| ++(1.5mm,0)|- (c\value.north);

\foreach \value in {1,2}
  \draw[-] (k2.south) -| ++(1.5mm,0)|- (l\value.north);
  
\foreach \value in {1,2,3}
  \draw[-] (c1.south) -| ++(1.5mm,0)|- (c1\value.west);

\foreach \value in {1,...,2}
  \draw[-] (c2.south) -| ++(1.5mm,0)|- (c2\value.north);

\foreach \value in {1,...,4}
  \draw[-] (c3.south) -| ++(1.5mm,0)|- (c3\value.west);

\foreach \value in {2,...,4}
  \draw[-] (c21.south) -| ++(1.5mm,0)|- (b\value.west);
  
\foreach \value in {1,...,3}
  \draw[-] (c22.south) -| ++(1.5mm,0)|- (d\value.west);

\foreach \value in {1,...,3}
    \draw[-] (c1\value.0) -| ++(1.5mm,0)|- (c1\value\value.west);

\foreach \value in {1,...,4}
    \draw[-] (c3\value.0) -| ++(1.5mm,0)|- (c3\value\value.west);

\foreach \value in {2,...,4}
    \draw[-] (b\value.0) -| ++(1.5mm,0)|- (b\value\value.west);

\foreach \value in {1,...,2}
    \draw[-] (e5\value.0) -| ++(1.5mm,0)|- (d2\value.west);
    
\foreach \value in {1,...,2}
    \draw[-] (d\value.0) -| ++(1.5mm,0)|- (d1\value.west);

\foreach \value in {1,...,2}
    \draw[-] (d3.0) -| ++(1.5mm,0)|- (e5\value.west);
\foreach \value in {1,...,5}
    \draw[-] (l1.south) -| ++(1.5mm,0)|- (l1\value.west);
\foreach \value in {1,...,2}
    \draw[-] (l2.south) -| ++(1.5mm,0)|- (l2\value.west);
\foreach \value in {1,...,5}
    \draw[-] (l1\value.0) -| ++(1.5mm,0)|- (l1\value\value.west);
\foreach \value in {1,...,2}
    \draw[-] (l2\value.0) -| ++(1.5mm,0)|- (l2\value\value.west);
\end{tikzpicture}
\caption{The way of organizing surveyed articles.}
\label{fig6}
\end{figure}

==> Table/table.tex <==
\begin{longtable}{c|c|c|c|c|c|c|c|c|c|c|c|c|c}

    \caption{Comparisons of LLM-based methods employed in in-context learning (ICL) and fine-tuning (FT) paradigms for text-to-SQL tasks. These methods are categorized based on their specific implementation designs: ICL-In-Context Learning, FT-Fine-Tuning, SL-Schema Linking, DCA-Database Content Acquisition, QR-Question Rewriting, DA-Data Augmentation, SKI-Supplementary Knowledge Incorporation, ES-Example Selection, RE-Reasoning Enhancement, FFT-Fully Fine-Tuning, PEFT-Parameter-Efficient Fine-Tuning, DC-Direct SQL Correction, EGC-Execution-Guided SQL Correction, OC-Output Consistency. Note that * indicates that various LLMs have been applied in the corresponding method, and we present the LLM showing the best performance in text-to-SQL tasks. Meanwhile, $\checkmark$ in the ES category shows that the corresponding method employs few-shot strategies.}
    \label{table:method} \\
			\toprule 
			\multirow{2}{*}{\scalebox{0.8}{\textbf{Methods}}} & \multirow{2}{*}{\scalebox{0.8}{\textbf{Applied LLMs}}} & \multicolumn{4}{c|}{\scalebox{0.8}{\textbf{Pre-Processing}}} & \multicolumn{3}{c|}{\scalebox{0.8}{\textbf{ICL}}} & \multicolumn{2}{c|}{\scalebox{0.8}{\textbf{FT}}} & \multicolumn{3}{c}{\scalebox{0.8}{\textbf{Post-Processing}}} \\ \cline{3-14} 
 &  & \scalebox{0.8}{SL} & \scalebox{0.8}{DCA} & \scalebox{0.8}{QR} & \scalebox{0.8}{DA} & \scalebox{0.8}{SKI} & \scalebox{0.8}{ES} & \scalebox{0.8}{RE} & \scalebox{0.8}{FFT} & \scalebox{0.8}{PEFT} & \scalebox{0.8}{DC} & \scalebox{0.8}{EGC} & \scalebox{0.8}{OC} \\
			\midrule 
			\endfirsthead
			
			\multicolumn{3}{l}%
			{{\bfseries-- Continued from previous page}} \\
			\hline 
            \multirow{2}{*}{\scalebox{0.8}{\textbf{Methods}}} & \multirow{2}{*}{\scalebox{0.8}{\textbf{Applied LLMs}}} & \multicolumn{4}{c|}{\scalebox{0.8}{\textbf{Pre-Processing}}} & \multicolumn{3}{c|}{\scalebox{0.8}{\textbf{ICL}}} & \multicolumn{2}{c|}{\scalebox{0.8}{\textbf{FT}}} & \multicolumn{3}{c}{\scalebox{0.8}{\textbf{Post-Processing}}} \\ \cline{3-14} 
 &  & \scalebox{0.8}{SL} & \scalebox{0.8}{DCA} & \scalebox{0.8}{QR} & \scalebox{0.8}{DA} & \scalebox{0.8}{SKI} & \scalebox{0.8}{ES} & \scalebox{0.8}{RE} & \scalebox{0.8}{FFT} & \scalebox{0.8}{PEFT} & \scalebox{0.8}{DC} & \scalebox{0.8}{EGC} & \scalebox{0.8}{OC}  \\ 
 \midrule 
			\endhead
			
			\midrule \multicolumn{3}{l}{{\bfseries-- Continued on next page}} \\ 
			\endfoot
			
			\midrule
			\endlastfoot
   
{\scalebox{0.8}{Rajkumar et al. \cite{rajkumar2022evaluating}}} & {\scalebox{0.8}{GPT-3.5}} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {} & {} & {}\\ 
   
{\scalebox{0.8}{C3 \cite{dong2023c3}}} & {\scalebox{0.8}{GPT-3.5}} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$}\\ 

{\scalebox{0.8}{DIN-SQL \cite{pourreza2024din}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {$\checkmark$} & {$\checkmark$} & {} & {} & {$\checkmark$} & {} & {}  \\ 

{\scalebox{0.8}{CRUSH4SQL \cite{kothyari2023crush4sql}}} & {\scalebox{0.8}{GPT-3.5*}} & {$\checkmark$} & {} & {$\checkmark$} & {} & {} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {} & {}\\ 

{\scalebox{0.8}{DESEM+P \cite{guo2023prompting}}} & {\scalebox{0.8}{GPT-3.5}} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {} & {} & {$\checkmark$} & {}\\ 

{\scalebox{0.8}{CHATDB \cite{hu2023chatdb}}} & {\scalebox{0.8}{GPT-3.5}} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {} & {$\checkmark$} & {} & {} & {} & {} & {}\\ 

{\scalebox{0.8}{SQL-PaLM \cite{sun2023sql}}} & {\scalebox{0.8}{PaLM-2}} & {$\checkmark$} & {$\checkmark$} & {} & {$\checkmark$} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$} & {}\\ 

{\scalebox{0.8}{ReBoostSQL \cite{sui2023reboost}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {} & {$\checkmark$} & {} & {} & {} & {} & {} & {} & {} & {$\checkmark$} & {}\\ 

{\scalebox{0.8}{Divide-and-Prompt \cite{liu2023divide}}} & {\scalebox{0.8}{GPT-3.5}} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {$\checkmark$} & {$\checkmark$} & {} & {} & {$\checkmark$} & {} & {}\\ 

{\scalebox{0.8}{LTMP-DA-GP \cite{arora2023adapt}}} & {\scalebox{0.8}{GPT-3.5*}} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {} & {}\\ 

{\scalebox{0.8}{DAIL-SQL \cite{gao2023text}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {} & {} & {$\checkmark$}\\ 

{\scalebox{0.8}{Nan et al. \cite{nan2023enhancing}}} & {\scalebox{0.8}{GPT-3.5*}} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {} & {} & {}\\ 

{\scalebox{0.8}{BINDER \cite{cheng2022binding}}} & {\scalebox{0.8}{Codex}} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {} & {} & {}\\ 

{\scalebox{0.8}{Tai et al. \cite{tai2023exploring}}} & {\scalebox{0.8}{Codex}} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {} & {}\\ 

{\scalebox{0.8}{Liu et al. \cite{liu2023comprehensive}}} & {\scalebox{0.8}{Codex}} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {} & {} & {} & {}\\

{\scalebox{0.8}{DBCopilot \cite{wang2023dbcopilot}}} & {\scalebox{0.8}{GPT-3.5}} & {$\checkmark$} & {} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {} & {}\\ 

{\scalebox{0.8}{ODIS \cite{chang2023selective}}} & {\scalebox{0.8}{GPT-3.5*}} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {} & {} & {}\\ 

{\scalebox{0.8}{Guo et al. \cite{guo2023retrieval}}} & {\scalebox{0.8}{Text-DaVinci}} & {$\checkmark$} & {} & {$\checkmark$} & {} & {$\checkmark$} & {} & {} & {} & {} & {} & {$\checkmark$} & {}\\ 

{\scalebox{0.8}{ZeroNL2SQL \cite{gu2023interleaving}}} & {\scalebox{0.8}{GPT-3.5}} & {$\checkmark$} & {} & {} & {} & {} & {} & {} & {} & {} & {} & {$\checkmark$} & {}\\ 

{\scalebox{0.8}{SQLPrompt \cite{sun2023sqlprompt}}} & {\scalebox{0.8}{GPT-3.5}} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {} & {} & {$\checkmark$}\\ 

{\scalebox{0.8}{LEVER \cite{ni2023lever}}} & {\scalebox{0.8}{Code-DaVinci*}} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {} & {} & {$\checkmark$}\\

{\scalebox{0.8}{Chang et al. \cite{chang2023prompt}}} & {\scalebox{0.8}{Code-DaVinci*}} & {} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {} & {} & {}\\

{\scalebox{0.8}{PET-SQL \cite{li2024pet}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {$\checkmark$} & {} & {} & {$\checkmark$} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$}\\ 

{\scalebox{0.8}{MAC-SQL \cite{wang2024mac}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {}\\ 

{\scalebox{0.8}{ACT-SQL \cite{zhang2023act}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {} & {}\\ 

{\scalebox{0.8}{DEA-SQL \cite{xie2024decomposition}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {}\\

{\scalebox{0.8}{PURPLE \cite{ren2024purple}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {} & {$\checkmark$}\\ 

{\scalebox{0.8}{METASQL \cite{fan2024metasql}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$}\\ 

{\scalebox{0.8}{DAC \cite{wang2024dac}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {}\\ 

{\scalebox{0.8}{MAG-SQL \cite{xie2024mag}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {}\\ 

{\scalebox{0.8}{Wu et al. \cite{wu2024need}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {} & {} & {} & {} & {} & {} & {} & {} & {} & {$\checkmark$} & {}\\

{\scalebox{0.8}{Shen et al. \cite{shen2024improving}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {} & {} & {}\\

{\scalebox{0.8}{TCSR-SQL \cite{xu2024tcsr}}} & {\scalebox{0.8}{GPT-3.5}} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {} & {}\\


{\scalebox{0.8}{SQLFixAgent \cite{cen2024sqlfix}}} & {\scalebox{0.8}{CodeS, GPT-3.5}} & {$\checkmark$} & {} & {} & {} & {} & {} & {} & {} & {} & {} & {$\checkmark$} & {}\\

{\scalebox{0.8}{MAGIC \cite{askari2024magic}}} & {\scalebox{0.8}{GPT-4}} & {$\checkmark$} & {} & {} & {} & {} & {} & {} & {} & {} & {} & {$\checkmark$} & {}\\ 

{\scalebox{0.8}{CHESS \cite{talaei2024chess}}} & {\scalebox{0.8}{{DeepSeek, GPT-3.5, GPT-4}}} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$} & {}\\ 

{\scalebox{0.8}{TA-SQL \cite{qu2024before}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {} & {} & {}\\ 

{\scalebox{0.8}{IntelliExplain \cite{yan2024intelliexplain}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {} & {$\checkmark$} & {} & {} & {} & {} & {} & {} & {} & {} & {}\\

{\scalebox{0.8}{MCS-SQL \cite{lee2024mcs}}} & {\scalebox{0.8}{GPT-4}} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {} & {} & {$\checkmark$}\\ 

{\scalebox{0.8}{EPI-SQL \cite{liu2024epi}}} & {\scalebox{0.8}{GPT-4}} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {} & {} & {}\\ 

{\scalebox{0.8}{Dubo-SQL \cite{thorpe2024dubo}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$} & {}\\

{\scalebox{0.8}{DFIN-SQL \cite{volvovsky2024dfin}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {} & {}\\

{\scalebox{0.8}{$\text{R}^3$ \cite{xia2024r3thissqlme}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$} & {}\\ 

{\scalebox{0.8}{FUSED \cite{wang2024improving}}} & {\scalebox{0.8}{GPT-3.5*}} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {} & {} & {}\\ 

{\scalebox{0.8}{Li et al. \cite{li2024using}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {} & {} & {} & {} & {} & {} & {} & {} & {} & {} & {$\checkmark$}\\ 

{\scalebox{0.8}{SELF-DEBUGGING \cite{chen2024teaching}}} & {\scalebox{0.8}{GPT-4*}} & {} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$} & {}\\

{\scalebox{0.8}{SGU-SQL \cite{zhang2024structure}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {} & {}\\

{\scalebox{0.8}{FUXI \cite{gu2024middleware}}} & {\scalebox{0.8}{GPT-4*}} & {} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$} & {}\\ 

{\scalebox{0.8}{DART-SQL \cite{mao2024enhancing}}} & {\scalebox{0.8}{GPT-3.5}} & {$\checkmark$} & {$\checkmark$} & {$\checkmark$} & {} & {} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$} & {}\\ 

{\scalebox{0.8}{Tool-SQL \cite{wang2024tool}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {} & {} & {} & {} & {} & {} & {} & {} & {} & {$\checkmark$} & {}\\ 

{\scalebox{0.8}{SEA-SQL \cite{li2024sea}}} & {\scalebox{0.8}{GPT-4*}} & {} & {} & {} & {} & {} & {} & {} & {} & {} & {} & {$\checkmark$} & {}\\ 

{\scalebox{0.8}{SL+CC \cite{tan2024enhancing}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$}\\

{\scalebox{0.8}{SELECT-SQL \cite{shen2024selectsql}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {$\checkmark$}\\

{\scalebox{0.8}{MLPrompt \cite{wang2024large}}} & {\scalebox{0.8}{GPT-4}} & {} & {} & {} & {} & {$\checkmark$} & {} & {$\checkmark$} & {} & {} & {$\checkmark$} & {} & {}\\

{\scalebox{0.8}{PTD-SQL \cite{luo2024ptdsql}}} & {\scalebox{0.8}{GPT-4*}} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {} & {}\\

{\scalebox{0.8}{E-SQL \cite{caferolu2024esql}}} & {\scalebox{0.8}{GPT-4o*}} & {$\checkmark$} & {} & {$\checkmark$} & {} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {} & {}\\ 

{\scalebox{0.8}{CHASE-SQL \cite{pourreza2024chasesql}}} & {\scalebox{0.8}{Gemini 1.5*}} & {$\checkmark$} & {$\checkmark$} & {} & {$\checkmark$} & {$\checkmark$} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {$\checkmark$}\\ 

{\scalebox{0.8}{AC-SQL \cite{zheng2024actor}}} & {\scalebox{0.8}{GPT-4o*}} & {} & {} & {} & {} & {} & {} & {} & {} & {} & {$\checkmark$} & {$\checkmark$} & {}\\ 

{\scalebox{0.8}{MARLO \cite{mai2024learning}}} & {\scalebox{0.8}{Llama 3-
70B-Instruct*}} & {} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {} & {} & {}\\ \midrule

{\scalebox{0.8}{CodeS \cite{li2024codes}}} & {\scalebox{0.8}{StarCoder}} & {$\checkmark$} & {$\checkmark$} & {} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {}\\

{\scalebox{0.8}{DTS-SQL \cite{pourreza2024dts}}} & {\scalebox{0.8}{DeepSeek*}} & {$\checkmark$} & {} & {} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {}\\

{\scalebox{0.8}{SQL-GEN \cite{pourreza2024sql}}} & {\scalebox{0.8}{CodeLlama}} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {}\\

{\scalebox{0.8}{SEA-SQL \cite{li2024sea}}} & {\scalebox{0.8}{Mistral-7B, GPT-3.5}} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {} & {} & {} & {$\checkmark$} & {} & {$\checkmark$} & {}\\

{\scalebox{0.8}{SENSE-SQL \cite{yang2024synthesizing}}} & {\scalebox{0.8}{{Deepseek-Coder, CodeLlama}}} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {}\\

{\scalebox{0.8}{SQLfuse \cite{zhang2024sqlfuse}}} & {\scalebox{0.8}{{Llama2, CodeFuse-DeepSeek}}} & {$\checkmark$} & {$\checkmark$} & {} & {} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {}\\

{\scalebox{0.8}{CCoE \cite{huang2024ccoe}}} & {\scalebox{0.8}{QWen1.5}} & {} & {} & {} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {}\\

{\scalebox{0.8}{DB-GPT-Hub \cite{zhou2024db2}}} & {\scalebox{0.8}{CodeLlama*}} & {} & {} & {} & {} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {}\\

{\scalebox{0.8}{Open-SQL \cite{chen2024open}}} & {\scalebox{0.8}{CodeLlama*}} & {$\checkmark$} & {} & {} & {} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {}\\

{\scalebox{0.8}{FinSQL \cite{zhang2024finsql}}} & {\scalebox{0.8}{LLaMA-2*}} & {$\checkmark$} & {} & {} & {$\checkmark$} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {}\\

{\scalebox{0.8}{Symbol-LLM \cite{xu2023symbol}}} & {\scalebox{0.8}{Symbol-LLM}} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {}\\

{\scalebox{0.8}{CLLMs \cite{kou2024cllms}}} & {\scalebox{0.8}{Deepseek}} & {} & {} & {} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {}\\

{\scalebox{0.8}{StructLM \cite{zhuang2024structlm}}} & {\scalebox{0.8}{CodeLlama}} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {}\\

{\scalebox{0.8}{YORO \cite{kobayashi2024yoro}}} & {\scalebox{0.8}{Mistral*}} & {} & {$\checkmark$} & {} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {}\\

{\scalebox{0.8}{DATAGPT-SQL \cite{wu2024datagptsql}}} & {\scalebox{0.8}{CodeQwen1.5}} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {$\checkmark$} & {} & {} & {$\checkmark$} & {}\\

{\scalebox{0.8}{ITERGEN \cite{ugare2024itergen}}} & {\scalebox{0.8}{Qwen2.5-Coder*}} & {} & {} & {} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {} & {}\\

{\scalebox{0.8}{MSc-SQL \cite{gorti2024msc}}} & {\scalebox{0.8}{Gemma-2-9B*}} & {$\checkmark$} & {} & {} & {} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {}\\

{\scalebox{0.8}{MoMQ \cite{lin2024momq}}} & {\scalebox{0.8}{Qwen1.5-14B*}} & {} & {} & {} & {} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {}\\

{\scalebox{0.8}{KID \cite{zhong2024learning}}} & {\scalebox{0.8}{QWen1.5-7B*}} & {} & {} & {} & {} & {} & {} & {} & {} & {$\checkmark$} & {} & {} & {}\\

\end{longtable}

